RGBD2lux: Dense light intensity estimation with an RGBD sensor

Lighting design and modelling or industrial applications like luminaire planning and commissioning rely heavily on time consuming manual measurements or on physically coherent computational simulations. Regarding the latter,standard approaches are based on CAD modeling simulations and offline rendering, with long processing times and therefore inflexible workflows. Thus, in this paper we pro-pose a computer vision based system to measure lighting with just a single RGBD camera. The proposed method uses both depth data and images from the sensor to provide a dense measure of light intensity in the field of view of the camera. We evaluate our system on novel ground truth data and compare it to state-of-the-art commercial light-planning software. Our system provides improved performance, while being completely automated, given that the CAD model is extracted from the depth and the albedo estimated with the support of RGB images. To the best of our knowledge, this is the first automatic framework for the estimation of lighting in general indoor scenarios from RGBDinput.

==> sections/evaluation_tuesdaynight_priortochanges.tex <==
\section{Experimental Evaluation} \label{sec:exps}

Experiments are organized as follows: Sec. \ref{sec:LMB} presents a novel dataset for light measurements; Sec. \ref{sec:luxcom} shows overall performance while Sec. \ref{sec:CADexp} describes in more details the evaluation of our radiosity model against state of the art approaches. Finally, Sec. \ref{sec:DEPTHexp} reports real experiments with the RGBD data only.

\subsection{Light measurement benchmark} \label{sec:LMB}

To the best of our knowledge, there is currently no dataset for benchmarking light measurements with ground truth in real scenes.  Thus, we define a new benchmark for light measurement in real world scenes. We select two different office rooms,% \ie two office rooms, 
 namely room\_1 and room\_2, see Figure \ref{fig:rooms1_full_scene}. As shown, we provide a detailed CAD design for the rooms representing the 3D ground truth. This includes an accurate labelling of the object textures and reflectivities for each surface facet in the CAD.

Both rooms have been equipped with a controlled lighting environment, since the position of eight luminaries is known (Fig \ref{fig:rooms1_full_scene}b), as well as their type (Siteco Mira), meaning that the LDC curve is given by the manufacturer. Furthermore, to achieve even more accurate ground truth, we measured in lab conditions the overall luminous flux and temperature of each luminaire being $7913lm$ and $4250k$ respectively, while the multiplicative parameter for the luminaire age\footnote{The efficiency of every luminaire degrades over time.} is assigned to value $1$ %(needed for the Relux simulations) 
since the installation is fairly new.

\begin{figure}[!ht]
	\begin{center}
	    \includegraphics[width=1\linewidth]{images/room1_all_no_gray_patches.png} %\hspace{.3cm}
% 		\includegraphics[width=0.48\linewidth]{images/render_room1_2.PNG} \\
% 		\textit{Room1}% \hspace{3cm} \textit{Room2}
	\end{center}
	\caption{Room\_1 full scene. (a) illustrate image as it looks from the camera, red bounding boxes are showing the location of luxmeters within the indoor space. Images (b) and (c) are detailed CAD design of the room showing the luminaire positioning and how the scene is scattered to individual patches respectively.} \label{fig:rooms1_full_scene}
% 	\vspace{-5pt}
\end{figure}

We provide for both rooms a number of sensory data. First, we set up in the ceiling of the rooms a RGBD calibrated and aligned sensory system which consists of an rgb camera with fish-eye lens with \ang{180} FOV and a depth camera (Bluetechnix time-of-flight) with \ang{90} FOV. However, in our experiments we consider only the part that is visible to both images after we have registered and undistorted them (as shown in Fig. \ref{fig:teaser} left).  %applied an undistortion pre-processing.

The sensors are synchronized with luxmeters (also indicated in Fig. \ref{fig:rooms1_full_scene}a and \ref{fig:rooms1_full_scene}b), %measuring  accurate illumination in lux and
providing therefore the ground truth data for illumination intensity. The luxmeters however give localized (\ie point-to-point) lux readings only, so we installed 8 of them  in different areas so providing a reasonable sampling of the environment. We chose mainly locations over desk areas, since they are of major importance in the lighting field. For each luxmeter, we additionally report the type and their specific light sensitivity characteristic curve (LSC, see Fig. \ref{fig:ldc_lsc}), namely the sensor sensitivity across the incident light angles.

Thereafter, we evaluate $31$ %different scenarios with 
different luminaire activations (luminaires switched on or off) for each room, see Fig. \ref{fig:illumination_combinations_room1} for a sample of  images obtained from room\_1. We target the use of rgb and depth input just for light measurement, the use of luxmeters as ground truth, and all other provided information for ablation studies.

\begin{figure}[ht!]
	\begin{center}
		\includegraphics[width=1\linewidth]{images/illumination_combinations1a.png}
	\end{center}
	\caption{Illustration of 4 illumination variants within room\_1. From the left, the images illustrate the illumination provided by 1, 3, 4 and all 8 luminaires switched on in the scene.}\label{fig:illumination_combinations_room1}
% 	\vspace{-15pt}
\end{figure}


\subsection{Quantitative comparisons in Lux}\label{sec:luxcom}

Table \ref{table:quantitative_room1_2} summarizes the overall performance of the commercial light modeling software Relux, compared to ours and both to the ground truth under all the different experimental inputs. Beyond the proposed RGBD2Lux, which does not require the CAD model and integrates the LDC and LSC curves, we additionally compare Relux to our own model using the CAD input provided (i.e. \textbf{Ours with CAD}). Results are reported for both room\_1 and room\_2.

Note that, when provided with the CAD model, our model outperforms Relux, thanks to the induced LDC and LSC distributions into the radiosity. In fact, against ground truth, \textbf{Ours CAD (LDC\_LSC)} achieves an average luxmeter error (across all 1-8 luxmeters) of $36$ Lux for room\_1 and $70$ Lux for room\_2\footnote{The supplemental material describes which are the structural differences between the two rooms together with the reason why room\_2 is more complex in terms of light modelling than room\_1}. These errors are $9.2\%$ and $3.7\%$ better than Relux, for room\_1 and room\_2 respectively.

Our proposed RGBD2Lux (modelling LDC and LSC but not requiring the CAD) is still comparable with the Relux (instead requiring the CAD). Here we only consider the luxmeters in the area visible from the depth-camera (\textbf{Avg (2-7)}), \ie those for which RGBD2Lux may compute a Lux value. For room\_1 we achieve an error of 61 Lux, and for room\_2 we achieve an error of 99 Lux. Thus, in this case the average lux error percentage is respectively worse than Relux by $4.6\%$ for room\_1, and by $8.1\%$ for room\_2.

It is of interest to note how the consideration of LSC provides a larger error reduction than LDC (rows 6 and 7 in the table), consistently across the two rooms. We interpret this as the way the form factors matrix is populated, \ie based on the ratio between the rays arriving at a patch by the overall emitted rays, where there is a higher dependency on the emitted rays rather than the received rays, %LDC being partly addressed in the Isocell ray-tracing and its distribution within the Isocell unit disc. By contract, LSC stands for modelling the sensor sensitivity and its dependency with the received rays, 
which would otherwise be equally strong from any angle.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!ht]
\centering
\caption{Illumination estimation errors by the considered approaches, applied to both rooms. Values for individual luxmeters, cols 1-8, correspond to the average lux values estimated over the results of the 31 different lighting combinations applied. Avg. (1-8) then to the average values of these for all installed luxmeters. By contrast, Avg. (2-7) only considers those luxmeters which are visible from the RGBD camera, \ie within its field-of-view. The percentage values correspond to the lux average percentage error in regards to the ground truth.}
\label{table:quantitative_room1_2}
\resizebox{.999\textwidth}{!}{\begin{tabu}{|c|c|c|c|c|c|c|c|c|c|c|l|c|c|c|c|c|c|c|c|c|c|}
\cline{1-11} \cline{13-22}
\multirow{3}{*}{\textbf{}}                                                                   & \multicolumn{10}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Room 1\\ Error (in Lux)\end{tabular}}}                                                                                                                                          &  & \multicolumn{10}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Room 2\\ Error (in Lux)\end{tabular}}}                                                                                                                                         \\ \cline{2-11} \cline{13-22} 
                                                                                             & \multicolumn{8}{c|}{\textbf{Luxmeters}}                                                               & \multicolumn{2}{c|}{\textbf{}}                                                                                                  &  & \multicolumn{8}{c|}{\textbf{Luxmeters}}                                                               & \multicolumn{2}{c|}{\textbf{}}                                                                                                 \\ \cline{2-11} \cline{13-22} 
                                                                                             & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{8} & \textbf{\begin{tabular}[c]{@{}c@{}}Avg.\\ (1-8)\end{tabular}}  & \textbf{\begin{tabular}[c]{@{}c@{}}Avg.\\ (2-7)\end{tabular}}  &  & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{8} & \textbf{\begin{tabular}[c]{@{}c@{}}Avg.\\ (1-8)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Avg.\\ (2-7)\end{tabular}}  \\ \cline{1-11} \cline{13-22} 
\textbf{Relux}                                                                               & 167        & 96         & 27         & 26         & 43         & 10         & 96         & 39         & \begin{tabular}[c]{@{}c@{}}63\\ (21.4\%)\end{tabular}          & \begin{tabular}[c]{@{}c@{}}50\\ (20.7\%)\end{tabular}          &  & 206        & 97         & 27         & 80         & 97         & 49         & 73         & 44         & \begin{tabular}[c]{@{}c@{}}84\\ (22.2\%)\end{tabular}         & \begin{tabular}[c]{@{}c@{}}71\\ (20.4\%)\end{tabular}          \\ \cline{1-11} \cline{13-22} 
\textbf{\begin{tabular}[c]{@{}c@{}}Ours with CAD\\ (no\_LDC\_LSC)\end{tabular}}              & 188        & 150        & 33         & 45         & 43         & 34         & 91         & 65         & \begin{tabular}[c]{@{}c@{}}81\\ (27.5\%)\end{tabular}          & \begin{tabular}[c]{@{}c@{}}66\\ (27.3\%)\end{tabular}          &  & 207        & 114        & 99         & 148        & 105        & 117        & 93         & 81         & \begin{tabular}[c]{@{}c@{}}120\\ (31.8\%)\end{tabular}        & \begin{tabular}[c]{@{}c@{}}112\\ (32.2\%)\end{tabular}         \\ \cline{1-11} \cline{13-22} 
\textbf{\begin{tabular}[c]{@{}c@{}}Ours with CAD\\ (LDC)\end{tabular}}                       & 199        & 152        & 29         & 41         & 40         & 33         & 95         & 57         & \begin{tabular}[c]{@{}c@{}}81\\ (27.5\%)\end{tabular}          & \begin{tabular}[c]{@{}c@{}}65\\ (26.9\%)\end{tabular}          &  & 213        & 117        & 82         & 125        & 97         & 97         & 86         & 63         & \begin{tabular}[c]{@{}c@{}}110\\ (29.1\%)\end{tabular}        & \begin{tabular}[c]{@{}c@{}}100\\ (28.8\%)\end{tabular}         \\ \cline{1-11} \cline{13-22} 
\textbf{\begin{tabular}[c]{@{}c@{}}Ours with CAD\\ (LSC)\end{tabular}}                       & 73         & 45         & 24         & 32         & 40         & 34         & 46         & 52         & \begin{tabular}[c]{@{}c@{}}43\\ (14.6\%)\end{tabular}          & \begin{tabular}[c]{@{}c@{}}37\\ (15.3\%)\end{tabular}          &  & 69         & 80         & 98         & 136        & 70         & 84         & 56         & 62         & \begin{tabular}[c]{@{}c@{}}82\\ (21.7\%)\end{tabular}         & \begin{tabular}[c]{@{}c@{}}87\\ (25.0\%)\end{tabular}          \\ \cline{1-11} \cline{13-22} 
\textbf{\begin{tabular}[c]{@{}c@{}}Ours with CAD\\ (LDC\_LSC)\end{tabular}}                  & 69         & 24         & 22         & 38         & 28         & 28         & 38         & 41         & \textbf{\begin{tabular}[c]{@{}c@{}}36\\ (12.2\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}30\\ (12.4\%)\end{tabular}} &  & 70         & 57         & 76         & 106        & 75         & 69         & 55         & 53         & \textbf{\begin{tabular}[c]{@{}c@{}}70\\ (18.5\%)\end{tabular}}  & \begin{tabular}[c]{@{}c@{}}73\\ (21.0\%)\end{tabular}          \\ \cline{1-11} \cline{13-22} 
\textbf{\begin{tabular}[c]{@{}c@{}}Ours with CAD\\ Camera visible\\ (LDC\_LSC)\end{tabular}} & -          & 64         & 28         & 20         & 17         & 22         & 52         & -          & -                                                              & \begin{tabular}[c]{@{}c@{}}34\\ (14.1\%)\end{tabular}          &  & -          & 54         & 36         & 59         & 101        & 69         & 54         & -          & -                                                             & \textbf{\begin{tabular}[c]{@{}c@{}}62\\ (17.8\%)\end{tabular}} \\ \cline{1-11} \cline{13-22} 
\textbf{\begin{tabular}[c]{@{}c@{}}Ours RGB2Lux\\ (LDC\_LSC)\end{tabular}}                   & -          & 53         & 41         & 67         & 68         & 40         & 98         & -          & -                                                              & \begin{tabular}[c]{@{}c@{}}61\\ (25.3\%)\end{tabular}          &  & -          & 98         & 90         & 85         & 136        & 108        & 77         & -          & -                                                             & \begin{tabular}[c]{@{}c@{}}99\\ (28.5\%)\end{tabular}          \\ \cline{1-11} \cline{13-22} 
\end{tabu}}
\end{table*}

\subsection{Comparisons against Relux using CAD models}
\label{sec:CADexp}

In the following, we detail the reasons why our system  performs better than the commercial Relux software \cite{relux} when the CAD model is available as input. We consider this as a sanity check (since Relux also uses radiosity) and we verify that our enriched model with the LDC and LSC curves reduce the estimation error against the ground truth readings from luxmeters. %For both systems, we consider the CAD as input since this information is needed for Relux to work (we would remove this input for the RGBD based evaluation in the next section).

Figure \ref{fig:rooms_full_scene_neg} shows six boxplots  of the light measurement error gathered across the $31$ different light scenarios for each luxmeter sesnsor. The x-axis represents each single luxmeter position with the numbering related to their position. %as shown in Figure \todo{\ref{xxx}} (as discussed, each luxmeter represents the ground truth measurement).
Each gray dot in the boxplot represents the error of a single light scenario, while the pink box in the boxplot represents the central 50\% of the data. Boxplot lower and upper boundary lines are at the 25\%-75\% quantile of the data. A central line indicates the median of the data, while the two vertical lines extending from the central box indicating the remaining data outside the central box that are regarded as outliers. These lines extend maximally to $1.5$ times the height of the pink box but not past the range of the data.

%\begin{figure}[!ht]
%	\begin{center}
%	    \includegraphics[width=1\linewidth]{images/illuminance_room1a.png} %\hspace{.3cm}
% 		\includegraphics[width=0.48\linewidth]{images/render_room1_2.PNG} \\
% 		\textit{Room1}% \hspace{3cm} \textit{Room2}
%	\end{center}
%	\caption{Room\_1 \& 2 lux error evaluation using the full CAD information against (a) Relux software, (b) standard radiosity model and (c) radiosity with \_LDC\_LSC applied.} \label{fig:rooms_full_scene}
% 	\vspace{-5pt}
%\end{figure}

\begin{figure}[!ht]
	\begin{center}
	    \includegraphics[width=1\linewidth]{images/illuminance_room1a.png} %\hspace{.3cm}
	   % \includegraphics[width=1\linewidth]{images/illuminance_d.png} %\hspace{.3cm}
% 		\includegraphics[width=0.48\linewidth]{images/render_room1_2.PNG} \\
% 		\textit{Room1}% \hspace{3cm} \textit{Room2}
	\end{center}
	\caption{Room\_1 \& 2 lux boxplot error evaluation using the full CAD information against (a) Relux software, (b) standard radiosity model and (c) radiosity with \_LDC\_LSC applied.} \label{fig:rooms_full_scene_neg}
% 	\vspace{-5pt}
\end{figure}

A global analysis of the results in Figure \ref{fig:rooms_full_scene_neg} shows that all the methods are under the median of $200$ lux error thus providing bounded results. This demonstrate as well that our customized radiosity model is at the level with state of the art solutions. When we apply the \_LDC\_LSC correction, our proposed radiosity model stands out clearly and it achieves better results than Relux. In particular, major reduction of the error happens at luxmeters 1, 2 and 7 for both room 1 and 2. In these three cases, the luxmeters are closely localized under the luminaries and ``looking'' directly at the light source (check Figure \ref{fig:rooms1_full_scene} for the geometrical distribution). At these positions, the error is due to a lower illuminance estimation by the radiosity model\footnote{See the signed plots in suppl. material}. Instead, these are cases of maximum light exposition and the LSC curve correctly model this phenomena coinciding with the luxmeter's sensitivity curve. Such improvement in performance  applies to both rooms.



Of particular interest is the case of luxmeter 4 for room 2 experiment, in that case neither the introduction of LSC and LDC can reduce the error. Figure \ref{fig:error_room2} shows the region where the luxmeter is located and it is quite revealing about what is causing this issue. For a set of light activations, there is a physical occlusion of a monitor screen casting a shadow over  luxmeter 4. In general a radiosity model shoud easily account this problem however due to such inaccuracies in the CAD design, \ie lack of the monitor screen for example in this case, we notice such discrepancies and higher errors in the evaluation of room two. 

\begin{figure}[!ht]
	\begin{center}
	    \includegraphics[width=1\linewidth]{images/img_004_room2a.png}
	\end{center}
	\caption{A detailed description of the problem for luxmeter 4 in room 2. There are higher errors due to  shadows on the luxmeter sensor and inaccuracy in the 3D CAD model. The graph plot next shows the correlation of the sensor's measurement and which light activation the error is a result of. }\label{fig:error_room2}
% 	\vspace{-5pt}
\end{figure}

%  \begin{figure}[thbp]
%  	\begin{center}
%  	    \includegraphics[width=.9\linewidth]{images/mesh_partial_room_reprojected.png}
%  	\end{center}
%  	\caption{The scene partially represented from only the areas that are visible to the camera FOV.}\label{fig:partial_room}
% % % 	\vspace{-5pt}
%  \end{figure}

% \begin{figure}[!ht]
% 	\begin{center}
% 	    \includegraphics[width=1\linewidth]{images/illuminance_room1_2_intersections.png}
% 	\end{center}
% 	\caption{ Room1 \& 2 Lux error evaluation using the visible CAD information for our method using radiosity with \_LDC\_LSC.}\label{fig:visible_scene}
% % 	\vspace{-5pt}
% \end{figure}

Before we move to the depth based simulations we established another experiment where we simulated a partial part of the CAD model.
% based on it alignment to the real scene (as shown in Figure Fig. \ref{fig:partial_room}). 
Here we simulate that the only CAD information available is the one actually visible by the camera. Such information might be available for instance to a depth camera observing the scene. In such case almost $60\%$ of the room is not visible so providing a real challenge for our light estimation system. Figure \ref{fig:visible_scene} shows the results for our radiosity with LDC\_LSC model  since i) it is the best performing against standard radiosity, ii) Relux software does not work with open surface (while we do). 

%  \begin{figure}[!ht]
%  	\begin{center}
%  	    \includegraphics[width=.8\linewidth]{images/mesh_partial_room_reprojected.png}
%  	\end{center}
%  	\caption{{\small The scene partially represented from only the areas that are visible to the camera FOV.}}\label{fig:partial_room}
% % % 	\vspace{-5pt}
%  \end{figure}

\begin{figure}[!ht]
	\begin{center}
	    \includegraphics[width=1\linewidth]{images/illuminance_room1_2_intersections.png}
	   % \includegraphics[width=1\linewidth]{images/illuminance_with_ldc_intersections_room1_2_neg.png}
	\end{center}
	\caption{ Room1 \& 2 Lux boxplot error evaluation using only the visible CAD information on the radiosity with \_LDC\_LSC.}\label{fig:visible_scene}
% 	\vspace{-5pt}
\end{figure}

Interestingly enough someone can notice the increment in the error for luxmeters 1, 2 and 8, especially in room 1, which are closer to the walls. Unfortunately since part of the walls are not visible because they are not included in the camera field of view the form factors fail to grasps the light contribution of the wall reflections, see Figure \ref{fig:visible_scene}.

% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[!ht]
% \centering
% \caption{Illumination estimation errors by the considered approaches, applied to both rooms. Values for individual luxmeters, cols 1-8, correspond to the average lux values estimated over the results of the 31 different lighting combinations applied. Avg. (1-8) then to the average values of these for all installed luxmeters. By contrast, Avg. (2-7) only considers those luxmeters which are visible from the depth-camera, \ie within its field-of-view.}
% \label{table:quantitative_room1_2}
% \resizebox{.999\textwidth}{!}{\begin{tabu}{|c|c|c|c|c|c|c|c|c|c|c|ll|c|c|c|c|c|c|c|c|c|c|}
% \cline{1-11} \cline{14-23}
% \multirow{3}{*}{}                                                                      & \multicolumn{10}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Room 1\\ Error (in Lux)\end{tabular}}}                                                                                                                                      &  &  & \multicolumn{10}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Room 2\\ Error (in Lux)\end{tabular}}}                                                                                                                                      \\ \cline{2-11} \cline{14-23} 
%                                                                                       & \multicolumn{8}{c|}{\textbf{Luxmeters}}                                                               & \multicolumn{2}{c|}{\textbf{}}                                                                                              &  &  & \multicolumn{8}{c|}{\textbf{Luxmeters}}                                                               & \multicolumn{2}{c|}{\textbf{}}                                                                                              \\ \cline{2-11} \cline{14-23} 
%                                                                                       & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{8} & \textbf{\begin{tabular}[c]{@{}c@{}}Avg.\\ (1-8)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Avg.\\ (2-7)\end{tabular}} &  &  & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{8} & \textbf{\begin{tabular}[c]{@{}c@{}}Avg.\\ (1-8)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Avg.\\ (2-7)\end{tabular}} \\ \cline{1-11} \cline{14-23} 
% \textbf{Relux}                                                                         & 167        & 96         & 27         & 26         & 43         & 10         & 96         & 39         & 63                                                           & 50                                                           &  &  & 206        & 97         & 27         & 80         & 97         & 49         & 73         & 44         & 84                                                           & 71                                                           \\ \cline{1-11} \cline{14-23} 
% \textbf{\begin{tabular}[c]{@{}c@{}}Ours with CAD\\ (no\_LDC\_LSC)\end{tabular}}               & 186        & 148        & 34         & 44         & 41         & 38         & 89         & 66         & 81                                                           & 66                                                           &  &  & 201        & 113        & 118        & 167        & 107        & 132        & 95         & 87         & 127                                                          & 122                                                          \\ \cline{1-11} \cline{14-23} 
% \textbf{\begin{tabular}[c]{@{}c@{}}Ours with CAD\\ (LDC)\end{tabular}}                      & 197        & 150        & 31         & 40         & 39         & 37         & 92         & 58         & 81                                                           & 65                                                           &  &  & 206        & 115        & 101        & 142        & 98         & 110        & 86         & 69         & 116                                                          & 108                                                          \\ \cline{1-11} \cline{14-23} 
% \textbf{\begin{tabular}[c]{@{}c@{}}Ours with CAD\\ (LSC)\end{tabular}}                      & 72         & 43         & 28         & 36         & 45         & 38         & 49         & 53         & 46                                                           & 40                                                           &  &  & 65         & 95         & 118        & 160        & 87         & 106        & 75         & 68         & 97                                                           & 106                                                          \\ \cline{1-11} \cline{14-23} 
% \textbf{\begin{tabular}[c]{@{}c@{}}Ours with CAD\\ (LDC\_LSC)\end{tabular}}                  & 69      & 22         & 23         & 42         & 33         & 32         & 41         & 41         & \textbf{38}                                                  & \textbf{32}                                                  &  &  & 67         & 70         & 93         & 129        & 74         & 82         & 70         & 58         & \textbf{80}                                                           & 86                                                           \\ \cline{1-11} \cline{14-23}%[-2.5pt] \tabucline[1.5pt]{1-11} \tabucline[1.5pt]{14-23}
%  \textbf{\begin{tabular}[c]{@{}c@{}}Ours with CAD\\ Camera visible\\ (LDC\_LSC)\end{tabular}} & -         & 64         & 27         & 20         & 17         & 22         & 52         & -         & -                                                           & 34                                                           &  &  & -         & 54         & 36         & 59         & 101        & 69         & 54         & -         & -                                                  & \textbf{62}                                                  \\[-2.5pt] \tabucline[1.5pt]{1-11} \tabucline[1.5pt]{14-23} 
% \textbf{\begin{tabular}[c]{@{}c@{}}Ours Depth2Lux\\ (LDC\_LSC)\end{tabular}}                                                                    & -          & 52         & 35         & 63         & 66         & 39         & 97         & -          & -                                                            & 59                                                           &  &  & -          & 99         & 86         & 85         & 129        & 107        & 79         & -          & -                                                            & 97                                                           \\ \cline{1-11} \cline{14-23} 
 
% \end{tabu}}
% \end{table*}

% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[!ht]
% \centering
% \caption{Illumination estimation errors by the considered approaches, applied to both rooms. Values for individual luxmeters, cols 1-8, correspond to the average lux values estimated over the results of the 31 different lighting combinations applied. Avg. (1-8) then to the average values of these for all installed luxmeters. By contrast, Avg. (2-7) only considers those luxmeters which are visible from the depth-camera, \ie within its field-of-view.}
% \label{table:quantitative_room1_2}
% \resizebox{.999\textwidth}{!}{\begin{tabu}{|c|c|c|c|c|c|c|c|c|c|c|ll|c|c|c|c|c|c|c|c|c|c|}
% \cline{1-11} \cline{14-23}
% \multirow{3}{*}{}                                                                      & \multicolumn{10}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Room 1\\ Error (in Lux)\end{tabular}}}                                                                                                                                      &  &  & \multicolumn{10}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Room 2\\ Error (in Lux)\end{tabular}}}                                                                                                                                      \\ \cline{2-11} \cline{14-23} 
%                                                                                       & \multicolumn{8}{c|}{\textbf{Luxmeters}}                                                               & \multicolumn{2}{c|}{\textbf{}}                                                                                              &  &  & \multicolumn{8}{c|}{\textbf{Luxmeters}}                                                               & \multicolumn{2}{c|}{\textbf{}}                                                                                              \\ \cline{2-11} \cline{14-23} 
%                                                                                       & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{8} & \textbf{\begin{tabular}[c]{@{}c@{}}Avg.\\ (1-8)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Avg.\\ (2-7)\end{tabular}} &  &  & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{8} & \textbf{\begin{tabular}[c]{@{}c@{}}Avg.\\ (1-8)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Avg.\\ (2-7)\end{tabular}} \\ \cline{1-11} \cline{14-23} 
% \textbf{Relux}                                                                         & 167        & 96         & 27         & 26         & 43         & 10         & 96         & 39         & 63                                                           & 50                                                           &  &  & 206        & 97         & 27         & 80         & 97         & 49         & 73         & 44         & 84                                                           & 71                                                           \\ \cline{1-11} \cline{14-23} 
% \textbf{\begin{tabular}[c]{@{}c@{}}Ours with CAD\\ (no\_LDC\_LSC)\end{tabular}}               & 188        & 150        & 33         & 45         & 43         & 34         & 91         & 65         & 81                                                           & 66                                                           &  &  & 207        & 114        & 99        & 148        & 105        & 117        & 93         & 81         & 120                                                          & 112                                                          \\ \cline{1-11} \cline{14-23} 
% \textbf{\begin{tabular}[c]{@{}c@{}}Ours with CAD\\ (LDC)\end{tabular}}                      & 199        & 152        & 29         & 41         & 40         & 33         & 95         & 57         & 81                                                           & 65                                                           &  &  & 213        & 117        & 82        & 125        & 97         & 97        & 86         & 63         & 110                                                          & 100                                                          \\ \cline{1-11} \cline{14-23} 
% \textbf{\begin{tabular}[c]{@{}c@{}}Ours with CAD\\ (LSC)\end{tabular}}                      & 73         & 45         & 24         & 32         & 40         & 34         & 46         & 52         & 43                                                           & 37                                                           &  &  & 69         & 80         & 98        & 136        & 70         & 84        & 56         & 62         & 82                                                           & 87                                                          \\ \cline{1-11} \cline{14-23} 
% \textbf{\begin{tabular}[c]{@{}c@{}}Ours with CAD\\ (LDC\_LSC)\end{tabular}}                  & 69      & 24         & 22         & 38         & 28         & 28         & 38         & 41         & \textbf{36}                                                  & \textbf{30}                                                  &  &  & 70         & 57         & 76         & 106        & 75         & 69         & 55         & 53         & \textbf{70}                                                           & 73                                                           \\ \cline{1-11} \cline{14-23}%[-2.5pt] \tabucline[1.5pt]{1-11} \tabucline[1.5pt]{14-23}
%  \textbf{\begin{tabular}[c]{@{}c@{}}Ours with CAD\\ Camera visible\\ (LDC\_LSC)\end{tabular}} & -         & 64         & 28         & 20         & 17         & 22         & 52         & -         & -                                                           & 34                                                           &  &  & -         & 54         & 36         & 59         & 101        & 69         & 54         & -         & -                                                  & \textbf{62}                                                  \\[-2.5pt] \tabucline[1.5pt]{1-11} \tabucline[1.5pt]{14-23} 
% \textbf{\begin{tabular}[c]{@{}c@{}}Ours Depth2Lux\\ (LDC\_LSC)\end{tabular}}                                                                    & -          & 53         & 41         & 67         & 68         & 40         & 98         & -          & -                                                            & 61                                                           &  &  & -          & 98         & 90         & 85         & 136        & 108        & 77         & -          & -                                                            & 99                                                           \\ \cline{1-11} \cline{14-23} 
 
% \end{tabu}}
% \end{table*}

\subsection{Light measurements from RGBD data} \label{sec:DEPTHexp}

To this end we evaluate the performance of RGBD2lux  using the RGBD data only and our customized radiosity model with \_LDC and \_LSC.

\begin{figure}[!ht]
	\begin{center}
	    \includegraphics[width=1\linewidth]{images/relux_rgbd2lux_room1.png}
	    \includegraphics[width=1\linewidth]{images/relux_rgbd2lux_room1_neg.png}
	\end{center}
	\caption{The figure shows the comparison between the Relux simulation with CAD model (left) and our RGBD2lux approach (right) for room\_1. Even if our method do not use the CAD model it achieves better or equivalent performance in some scenarios. Plots in the second row specify the type of the error, \ie due to lower \textit{(red marker)} or over \textit{(green marker)} estimation.}\label{fig:depth_illuminance_room1}
 	\vspace{-5pt}
\end{figure}

The boxplots in Figure \ref{fig:depth_illuminance_room1} shows that RBGD2lux achieves better or equivalent performance than the Relux simulation in some of the $31$ lighting scenarios tested. Note that in the estimated results with the depth input the error is mainly due to lower estimation of the illumination levels within the room as a cause of the missing geometry. However, considering also the incomplete geometry, this experiment shows that even with partial geometry information given by a depth sensor our system can perform or even overcome the CAD-based (with full geometry given) state of the art in challenging scenarios (similar results are obtained for room\_2 and they are presented in the supplemental material).

==> sections/introduction.tex <==
\section{Introduction} \label{sec:introduction}

In the industrial-driven process of creating and selling lighting concepts, the two aspects of light planning and lighting design rely heavily on physically reliable simulations and visualizations and both aspects has recently received increased scientific attention \cite{lin2013, schwarz2014, sorger2016}. Moreover, it has been shown that in a virtual environment this design process can be carried out in a completely interactive way using novel methods from the field of Visual Computing \cite{hilite,litemaker}. 

It is the fact though that only computationally expensive offline rendering algorithms are sufficiently accurate to capture complex effects of lighting modeling and simulation processes, which results in a costly and time-consuming development. Moreover, all these offline light modeling simulations are based on artificial designed CAD models of a scene and to data that need to be predefined or retrieved from online libraries, without representing accurately the exact real properties of the scene.

On the other hand the only hardware based alternative for capturing such complex lighting effects rely on the use of conventional lighting measurement sensors, \eg luxmeters, which are normally hand-held and feature what is known as point-to-point measurements. Meaning that the operator needs to repeat the measurement several times, swaying for angular and spatial completeness and as a consequence turning out in a very time and cost-expensive procedure.

\begin{figure*}[!ht]
	\begin{center}
	    \includegraphics[width=1\linewidth]{images/teaser3.png}
	\end{center}
	\caption{}\label{fig:teaser}
 	\vspace{-5pt}
\end{figure*}

These shortcomings as well as the advances in lighting design and computational imaging have created the conditions for a camera-aided process in the field of light design,modeling and analysis: This would not only combine interactive modeling, immediate simulation and real-time visualization during the luminaire planning process, but it would also allow coupling it with interactive lighting management, making it possible for a smart lighting system to adjust the internal parameters and therefore the light distribution behavior of a luminaire based on the spatial lighting estimation over time in real conditions - \textit{\textbf{imagine being able to detect dense spatial illumination inaccuracies and adjust the luminaires for maintaining the proper illumination levels according to predefined scenarios or ISO standards for quality living, working, agriculture, \etc environments}}. One of the major challenges in reaching this goal is to maintain physical correctness (a requirement in any light-modeling application) while introducing a camera-aided input.

In this paper, we therefore introduce a baseline study that combines light modeling and computational imaging and tries to evaluate the spatial light distribution of a (or multiple) light source, based on the geometry (one of the key elements to every lighting simulation process) obtained from a depth sensor. We propose the first system, RGBD2lux, for measuring the spatial illumination of a scene (see Figure 1), based on a depth camera installed in the ceiling and replacing the room geometry with the depth measurements. The system exploits a radiosity model, which includes the light distribution curve of the light sources (the radiation maps of the luminaires) and the light sensitivity curve of the measuring sensors (how the incident light angle influences the luxmeter readings).

We test our system on the acquired depth measurements of two office scenes with different structure, while for both scenes we manually label the objects and their reflectivity. Thereafter we compare our results to the ground truth measured illumination in the rooms (obtained by a number of luxmeters, which we have installed at various fixed spots) as well as to the corresponding offline simulations from a commercial lighting simulation software with the corresponding CAD-design geometry. The results through ablation studies show that indeed replacing key element parts of an offline lighting simulation process (geometry in this case) with ones retrieved from an online cameras system can sufficiently and reliable challenge the former by maintaining or even outperforming the needed physical correctness.

The rest of the paper is organized as follows: in Section \ref{sec:radiosity_model} we first introduce radiosity for light modeling; in Section \ref{sec:depth2lux} we describe its extension to light distribution and sensitivity curves, and the proposed use of depth-aided for light measurements; in Section \ref{sec:exps} we introduce the benchmark and conduct experiments and ablation studies; finally we conclude the paper in Section \ref{sec:conclusion}. Next we review related work.

==> sections/preliminaries.tex <==
\section{Application Overview} \label{sec:radiosity_model}

In this work, We introduce our indoor camera-aided light modeling for real scenes. Our application, as shown in Figure \ref{fig:teaser}, consists of two major part: the light modeling itself and its modification so that to be possible to address a real indoor environment. Both parts are based on radiosity and its application for representing the global scene illumination. We chose radiosity in contrast to more advanced and sophisticated approaches, see Section \ref{sec:visual_computing}, due to its simplicity, efficiency as well as because it is still the state-of-art in all commercial lighting simulation software in the lighting field (Relux, DIALux, AGi32). 
%To ease the description, we assume that the environment description is given by a complete CAD model.



==> sections/radiosity_revisited.tex <==
\section{Radiosity Revisited - RGBD2Lux} \label{sec:depth2lux}

Here we first extend Radiosity to model the light distribution curve (LDC) of light sources and the light sensitivity curves (LSC) of the measurement sensor. Then we introduce Radiosity modelling based on a RGBD camera input just, and removing the necessity of CAD designs.

\subsection{Customizing radiosity for real environments} \label{sec:inddor_lighting}

The radiosity model in Eq. \eqref{eq:radiosity_matrix} has two limitations: it assumes point light sources and it disregards the light perception. We address both aspects in our model extension, by introducing the LDC (for considering any light source) and the LSC (to model the light observer / sensor perception).

\begin{figure}[thbp]
	\begin{center}

		\subfloat[][]{\includegraphics[width=0.3\linewidth]{images/ldc_lsc1.png}\label{ldc_lsc}\label{fig:ldc_lsc}}
		\hspace{0.01em}
		\subfloat[][]{\includegraphics[width=0.35\linewidth]{images/ldc_unitsphere.png}\label{fig:isocell_3d_weighted}}
		\hspace{0.01em}
		\subfloat[][]
		{\includegraphics[width=0.32\linewidth]{images/unit_sphere_over_cad.png}\label{fig:isocel_rays}}
        \vspace{5pt}
		\caption{(\textit{a}) Radial representation of LDC and LSC curves, illustrating how both quantities are attenuated (radius) with the growing light incident angle (radial angle); (\textit{b}) weighted ray distribution of the Isocell unit sphere for LDC, heatmap-color-coded; (\textit{c}) Isocell unit sphere (blue hemisphere) for a patch on the floor of the office CAD. The color-dots in (\textit{c}) are taken from (\textit{b}) but placed at the intersection of the cast ray with the other scene patches.} % \textcolor{blue}{TODO: if there is time replace first two subimages}}
		\label{fig:weighted_rays}
	\end{center}
% 	\vspace{-15pt}
\end{figure}

\paragraph{Light distribution curve (LDC).} Let us recall Equations \eqref{eq:radiosity} and \eqref{eq:radiosity_matrix}. The radiosity model uses a scalar variable $e_i$ to set whether each patch is a light source ($e_i>0$) or not ($e_i=0$). The actual $e_i$ value would relate to the radiant intensity or luminous flux of the light source, measured in lumens $[cd/sr]$. Since it uses scalar values, the Radiosity formulation of Section \ref{sec:radiosity_model} assumes isotropic light sources, \ie active patches radiate with the same intensity in all direction.

%If we are not interested to know the exact radiosity in the unit measure, we can assign a value of $1$ for an active patch and $0$ otherwise. 
%Likewise, the reflectivity value $\rho$ can be assigned at each patch in the CAD model. This procedure is  well automatized by light modelling software toolboxes \cite{relux,dialux} that provides a reflectance value given different furniture and surface in residential and office like environments. 

But isotropy is hardly the case for real light sources which are normally represented by a radiation map, such as in Figure \ref{fig:ldc_lsc} (\textit{red}). Their distribution is in general non-linear and encoded in a light distribution curve which provides the radiant intensity with respect to distance and angle from the emitting source (\ie how much light is emitted in each direction). The LDC curves are obtained experimentally in lab environment conditions with the use of specific equipment, \ie goniophotometer, and provided in datasheets by the luminaire manufacturer.

Thus, similarly to the existing solutions we include the LDC curve into the ray tracking procedure of our application and therefore we encode the non-linear radiation of light sources into the form factors $f_{ij}$. In more detail, we associate scalar values to each light source patch cast ray, which are proportional to the angle of emission, as illustrated in Figure \ref{fig:isocell_3d_weighted}. These are then used to re-write Eq. \eqref{eq:ratio} as a weighted mean. Since this procedure encodes the non-linear LDC into the form factors, our re-formulation of Radiosity preserves the linearity of Eq. \eqref{eq:radiosity_matrix}.

Note that, in this way, the non-linearity is embedded in the form factor computation process, which is already non-linear. This results therefore in a minimal impact on computation, since the system in Eq. \eqref{eq:radiosity_matrix} remains linear.

% \begin{equation} \label{eq:ratio_ldc}
%     m_j = \sum (\frac{m_i * m_{j_{LDC}}}{\sum (m_{i_{LDC}})}),
% \end{equation}

% where $LDC_j$ are the weighted values corresponding to the rays reaching to patch $j$ and $LDC_r$ are all the weigthed values emmiting from patch $i$



\paragraph{Light sensitivity curve (LSC).} People perceive light differently, depending on their orientation with respect to it (whether they are frontally illuminated or from the side) and depending on the distance from it.

In a similar fashion, luxmeter sensors have different sensitivity to lighting, depending on the lighting angle and distance. The LSC plot in Figure \ref{fig:ldc_lsc} (\textit{blue}) illustrates the detail perception characteristic of the luxmeter which we adopt in order to meet the measuring requirements of the collected ground truth data. Note the strong similarities to the discussed LDC in Figure \ref{fig:ldc_lsc} (\textit{red}).

Therefore, we correct the sensor's light perception by the LSC. Similarly to the LDC, we formulate the corresponding weighted Isocell unit sphere, as in Figure \ref{fig:isocell_3d_weighted}, and integrate the weights into the form factor calculation by modifying the ray casting. In this way, we maintain the Radiosity linear formulation and alter the computation time minimally. It is worth mentioning here that this functionality is not possible to be applied in any of the commercial light planning software.

\subsection{Camera-aided radiosity}

Most simulated environments need the a priori information of the CAD model. This is often hard to obtain in every lighting setup scenario and, when CAD is available, it is common to contain structural inaccuracies of the environment. To this end in this work we look on the problem from another perspective and we examine a pipeline to use a depth-camera to obtain reliable light measurements without using a CAD model but a sensor based retrieved geometry instead. The main goal here is to reconstruct the surface from the point cloud and represent it as a pair of vertices and faces. 

% \begin{figure*}[thbp]
% 	\begin{center}
% 	    \includegraphics[width=1\linewidth]{images/all_pipe_line_pt_cloud.png} %\hspace{.3cm}
% % 		\includegraphics[width=0.48\linewidth]{images/render_room1_2.PNG} \\
% % 		\textit{Room1}% \hspace{3cm} \textit{Room2}
% 	\end{center}
% 	\caption{(a) Initial point cloud; (b) mesh given by the Delaunay triangulation; (c) Laplacian smoothing; (d) Extracted faces from the mesh.} \label{fig:all_pipe_line_pt_cloud}
% % 	\vspace{-5pt}
% \end{figure*}

However, the main issues to deal with is that depth sensors provide a sparse and noisier point cloud from which it is difficult to obtain a complete CAD like representation. Thus, given an exemplar point cloud, we first apply a denoising procedure so that to remove any outlier points, we then apply a mesh reconstruction solution based on the poison surface reconstruction approach and finally we smooth the mesh with a Laplacian filter before we use the extracted faces as the needed patches for the form factors computation. % from where we throw rays into the space.

Thereafter, we specify the light source position in 3D. We assume this information is known, as luminaires may hardly be moved after their installation. The reflectance, $\rho$, values of surface are assigned based on a photometric stereo solution where the individual light sources activated RGB images were used accordingly. Then these values were mapped to the surface faces as the mean value of the pixels, of the albedo map image, falling within the area of each triangle.

% manually after we extracted and labeled each surface of our 3D model to individual materials and objects (we used online libraries likewise to the other commercial light planning software).

The procedure for obtaining a CAD models from depth data provides a coarse mesh, thus we want to examine whether it is sufficient for generating reliable lighting measures as shown in the experimental section. This is simply done by solving the same least-squares estimate of the radiosity model in order to obtain the values $\vec r$ from Eq. \eqref{eq:radiosity_matrix}. 

Lastly another aspect is that the surface we obtain in this case it is likely to be open since the depth camera observes a partial portion of the room and certainly it cannot perceive the structure of the ceiling. This partial 3D model is not usable by most commercial lighting software, which request a complete closed 3D model instead. Our radiosity  model can simply deal with this problem by applying a closure procedure \cite{vanLeersum1989} where Leersum’s rectification spreads the closure adjustments over all of the calculated view factors matrix values. After forming (\ref{eq:radiosity_matrix}), solving the linear system provides the light measurement at each patch.
